Impact of spatial transformations on landscape features of CEC2022 basic benchmark problems

When benchmarking optimization heuristics, we need to take care to avoid an algorithm exploiting biases in the construction of the used problems. One way in which this might be done is by providing different versions of each problem but with transformations applied to ensure the algorithms are equipped with mechanisms for successfully tackling a range of problems. In this paper, we investigate several of these problem transformations and show how they influence the low-level landscape features of a set of 5 problems from the CEC2022 benchmark suite. Our results highlight that even relatively small transformations can significantly alter the measured landscape features. This poses a wider question of what properties we want to preserve when creating problem transformations, and how to fairly measure them.

==> input/ela_list.tex <==
\begin{table}[h]
    \centering
    \caption{Selected ELA features' detailed names in \textit{flacco}.\dv{I think we can drop this table}
    % \ak{I think this can go to the appendix}
    }
    % \begin{subtable}[h]{0.32\textwidth}
        \centering
        % \scalebox{1}{
        \begin{tabular}{@{}l@{}}
        \toprule
        detailed names               \\ \midrule
        disp.ratio\_mean\_02         \\
        disp.ratio\_mean\_05         \\
        disp.ratio\_mean\_10         \\
        disp.ratio\_mean\_25         \\
        disp.ratio\_median\_02       \\
        disp.ratio\_median\_05       \\
        disp.ratio\_median\_10       \\
        disp.ratio\_median\_25       \\
        disp.diff\_mean\_02          \\
        disp.diff\_mean\_05          \\
        disp.diff\_mean\_10          \\
        disp.diff\_mean\_25          \\
        disp.diff\_median\_02        \\
        disp.diff\_median\_05        \\
        disp.diff\_median\_10        \\
        disp.diff\_median\_25        \\
        ela\_distr.skewness          \\
        ela\_distr.kurtosis          \\
        ela\_distr.number\_of\_peaks \\
    %     \bottomrule
    %     \end{tabular}
    %     }
    % \end{subtable}
    % \begin{subtable}[h]{0.32\textwidth}
    %     \centering
    %     \scalebox{1}{
    %     \begin{tabular}{@{}l@{}}
    %     \toprule
    %     detailed name                \\ \midrule
        ela\_level.mmce\_lda\_10     \\
        ela\_level.mmce\_qda\_10     \\
        ela\_level.lda\_qda\_10      \\
        ela\_level.mmce\_lda\_25     \\
        ela\_level.mmce\_qda\_25     \\
        ela\_level.lda\_qda\_25      \\
        ela\_level.mmce\_lda\_50     \\
        ela\_level.mmce\_qda\_50     \\
        ela\_level.lda\_qda\_50      \\
        ela\_meta.lin\_simple.adj\_r2           \\
        ela\_meta.lin\_simple.intercept         \\
        ela\_meta.lin\_simple.coef.min          \\
        ela\_meta.lin\_simple.coef.max          \\
        ela\_meta.lin\_simple.coef.max\_by\_min \\
        ela\_meta.lin\_w\_interact.adj\_r2      \\
        ela\_meta.quad\_simple.adj\_r2          \\
        ela\_meta.quad\_simple.cond             \\
        ela\_meta.quad\_w\_interact.adj\_r2     \\ 
        ic.h\_max                               \\
    %     \bottomrule
    %     \end{tabular}
    %     }
    % \end{subtable}
    % \begin{subtable}[h]{0.32\textwidth}
    %     \centering
    %     \scalebox{1}{
    %     \begin{tabular}{@{}l@{}}
    %     \toprule
    %     detailed name                           \\ \midrule
        ic.eps\_s                               \\
        ic\_eps.max                             \\
        ic.eps\_ration                          \\
        ic.m0                                   \\
        nbc.nn\_nb.sd\_ratio                    \\
        nbc.nn\_nb.mean\_ratio                  \\
        nbc.nn\_nb.cor                          \\
        nbc.dist\_ratio.coeff\_var              \\
        nbc.nb\_fitness.cor                     \\
        pca.expl\_var.cov\_x                    \\
        pca.expl\_var.cor\_x                    \\
        pca.expl\_var.cov\_init                 \\
        pca.expl\_var.cor\_init                 \\
        pca.expl\_var\_PC1.cov\_x               \\
        pca.expl\_var\_PC1.cor\_x               \\
        pca.expl\_var\_PC1.cov\_init            \\
        pca.expl\_var\_PC1.cor\_init            \\
        % \\ 
        % \\ 
        \bottomrule
        \end{tabular}
        % }
    % \end{subtable}
    \label{tab:ela_list}
\end{table}

==> input/x_pvalue_wd.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/x_translation/pvalue.eps}
        \caption{}
        \label{fig:subtract_pvalue}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/x_translation/wd.eps}
        \caption{}
        \label{fig:subtract_wd}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/x_scaling/pvalue.eps}
        \caption{}
        \label{fig:scale_pvalue}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/x_scaling/wd.eps}
        \caption{}
        \label{fig:scale_wd}
    \end{subfigure}
    \caption{\ak{update this caption}}
    \label{fig:x_pvalue_wd}
\end{figure*}

==> input/y_pvalue_wd.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/y_translation/pvalue.eps}
        \caption{}
        \label{fig:y_subtact_pvalue}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/y_translation/wd.eps}
        \caption{}
        \label{fig:y_subtact_wd}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/y_scaling/pvalue.eps}
        \caption{}
        \label{fig:y_scale_pvalue}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\linewidth}
        \includegraphics[width=\linewidth,trim=3mm 4mm 3mm 3mm,clip]{figs/y_scaling/wd.eps}
        \caption{}
        \label{fig:y_scale_wd}
    \end{subfigure}
    \caption{\ak{is this the same as figure 2?} }
    \label{fig:y_pvalue_wd
    }
\end{figure*}
